Rethinking Generalization: The Impact of Annotation Style on Medical Image Segmentation

Generalization is an important attribute of machine learning models, particularly for those that are to be deployed in a medical context, where unreliable predictions can have real world consequences. While the failure of models to generalize across datasets is typically attributed to a mismatch in the data distributions, performance gaps are often a consequence of biases in the 'ground-truth' label annotations. This is particularly important in the context of medical image segmentation of pathological structures (e.g. lesions), where the annotation process is much more subjective, and affected by a number underlying factors, including the annotation protocol, rater education/experience, and clinical aims, among others. In this paper, we show that modeling annotation biases, rather than ignoring them, poses a promising way of accounting for differences in annotation style across datasets. To this end, we propose a generalized conditioning framework to (1) learn and account for different annotation styles across multiple datasets using a single model, (2) identify similar annotation styles across different datasets in order to permit their effective aggregation, and (3) fine-tune a fully trained model to a new annotation style with just a few samples. Next, we present an image-conditioning approach to model annotation styles that correlate with specific image features, potentially enabling detection biases to be more easily identified.

==> Makefile <==
CC = latexmk
CFLAGS = -use-make -pdflatex -silent -time

.PHONY: all clean FORCE

MAINDIR = ..

PDFS = $(MAINDIR)/melba-sample-accepted-special-issue.pdf \
	$(MAINDIR)/melba-sample-accepted.pdf \
	$(MAINDIR)/melba-sample-in-submission.pdf \
	$(MAINDIR)/melba-sample-arxiv-submission.pdf \
	$(MAINDIR)/melba-sample.pdf


all: $(PDFS)

melba.sty: $(MAINDIR)/melba.sty
	cp $< $@

sample.bib: $(MAINDIR)/sample.bib
	cp $< $@

melba-sample-%.tex: $(MAINDIR)/melba-sample.tex melba-sample-%.patch
	patch $^ -o $@

$(MAINDIR)/melba-sample-%.pdf: melba-sample-%.tex melba.sty sample.bib FORCE
	$(CC) $(CFLAGS) $<
	cp $(@F) $@

$(MAINDIR)/melba-sample.pdf: $(MAINDIR)/melba-sample.tex melba.sty FORCE
	$(CC) $(CFLAGS) $<
	cp $(@F) $@


clean:
	rm -f *.aux *.bbl *.blg *.log *.fls *.fdb_latexmk
	rm -f melba-sample-*.tex
	rm -f *.out
	rm -f *.tex melba.sty sample.bib

FORCE:

